Mean field control problems for vaccine distribution

With the invention of the COVID-19 vaccine, shipping and distributing are crucial in controlling the pandemic. In this paper, we build a mean-field variational problem in a spatial domain, which controls the propagation of pandemic by the optimal transportation strategy of vaccine distribution. Here we integrate the vaccine distribution into the mean-field SIR model designed in our previous paper arXiv:2006.01249. Numerical examples demonstrate that the proposed model provides practical strategies in vaccine distribution on a spatial domain.

==> Vaccine MFG/tmp_main_header.tex <==
\title{Mean field control problems for Vaccine distribution\thanks{Submitted to the editors \today
\funding{This work is supported by AFOSR MURI FA9550-18-1-0502.}}}

\author{{Wonjun Lee}
\thanks{Department of Mathematics, University of California, Los Angeles (\email{wlee@math.ucla.edu}, \email{siting6@math.ucla.edu},  \email{sjo@math.ucla.edu.})}
\and {Siting Liu}\footnotemark[2]
\and {Wuchen Li}
\thanks{Department of Mathematics, University of South Carolina (\email{wuchen@mailbox.sc.edu})}
\and {Stanley Osher}\footnotemark[2]}

\headers{Mean field control problems for vaccine distribution}{Lee, Liu, Li and Osher}

